Depends-Kotlin: A Cross-Language Kotlin Dependency Extractor

Since Google introduced Kotlin as an official programming language for developing Android apps in 2017, Kotlin has gained widespread adoption in Android development. However, compared to Java, there is limited support for Kotlin code dependency analysis, which is the foundation to software analysis. To bridge this gap, we develop Depends-Kotlin to extract entities and their dependencies in Kotlin source code. Not only does Depends-Kotlin support extracting entities' dependencies in Kotlin code, but it can also extract dependency relations between Kotlin and Java. Using three open-source Kotlin-Java mixing projects as our subjects, Depends-Kotlin demonstrates high accuracy and performance in resolving Kotlin-Kotlin and Kotlin-Java dependencies relations. The source code of Depends-Kotlin and the dataset used have been made available at https: //github.com/XYZboom/depends-kotlin. We also provide a screen-cast presenting Depends-Kotlin at https://youtu.be/ZPq8SRhgXzM.

==> table_extracted_deps.tex <==
\begin{table*}[!tbp]
    \centering
    \small
    \caption{Dependency Relations Extracted by \textit{Depends-Kotlin}}
    \label{tbl:extracted-deps}
    \begin{tabular}{c|cccc|cccc|cccc||c}
    \hline
       \multirow{2}{*}{}  & \multicolumn{4}{|c|}{\textbf{DSU-Sideloader}}  & \multicolumn{4}{|c|}{\textbf{Flap}} & \multicolumn{4}{|c||}{\textbf{RootEncoder}} & \multirow{2}{*}{\textbf{Total}}   \\ \cline{2-13}
         & K-J & J-K & K-K & J-J & K-J & J-K & K-K & J-J & K-J & J-K & K-K & J-J  \\ \hline
        Import & 19 & 0 & 170 & 1 & 3 & 0 & 170 & 1 & 102 & 190 & 913 & 193 & 1762 \\ \hline
        Contain & 6 & 0 & 34 & 5 & 4 & 0 & 46 & 63 & 10 & 256 & 318 & 73  & 815 \\ \hline
        Extend & 1 & 0 & 4 & 0 & 0 & 0 & 20 & 2 & 6 & 1 & 101 & 75  & 210 \\ \hline
        Implement & 1 & 0 & 0 & 7 & 0 & 0 & 36 & 1 & 9 & 4 & 8 & 3 & 69 \\ \hline
        Call & 50 & 0 & 450 & 81 & 3 & 0 & 370 & 479 & 62 & 423 & 1278 & 1316 & 4512 \\ \hline
        Create & 1 & 0 & 31 & 2 & 3 & 0 & 94 & 25 & 59 & 71 & 489 & 57 & 832 \\ \hline
        Cast & 0 & 0 & 0 & 1 & 5 & 0 & 10 & 15 & 0 & 8 & 48 & 9 & 96 \\ \hline
        Annotation & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 2 & 0 & 0 & 0 & 0 & 2 \\ \hline
        Use & 70 & 0 & 703 & 187 & 9 & 0 & 713 & 1093 & 141 & 203 & 3331 & 4317 & 10767  \\ \hline
        Parameter & 1 & 0 & 48 & 9 & 0 & 0 & 40 & 46 & 29 & 121 & 238 & 145  & 677 \\ \hline
        Return & 3 & 0 & 36 & 16 & 0 & 0 & 71 & 24 & 2 & 30 & 263 & 30 & 475 \\ \hline
        Delegate & 0 & - & 0 & - & 0 & - & 2 & - & 0 & - & 0 & - & 2 \\ \hline
        Extension & 0 & - & 0 & - & 0 & - & 6 & - & 0 & - & 3 & - & 9 \\ \hline \hline
        \textbf{Total} & 152 & 0 & 1476 & 309 & 27 & 0 & 1578 & 1751 & \cellcolor{gray!60} 420 & \cellcolor{gray!60} 1307 & 6990 & 6218 \\ \hline
    \end{tabular}
\end{table*}

==> table_projects.tex <==

\begin{table}[!tbp]
    \centering
    \small
    \caption{Our Study Subjects}
    \label{tbl:subjects}
    \vspace{-4mm}
    \begin{tabular}{ccccc}
     \hline
     \toprule
        \textbf{ProjectName} & \textbf{\#Stars } & \textbf{Kotlin(\%)} & \textbf{Java(\%)} 
        & \textbf{\#LOC} \\ 
         \midrule
{\sffamily DSU-Sideloader} & 1259 & 94.1 & 4.5 & 7k    \\
{\sffamily Flap}  & 286 & 52.4 & 47.6  & 16k   \\
{\sffamily RootEncoder} & 738 & 55.8 & 42.1 & 51k \\
         \bottomrule
    \end{tabular}
\end{table}
